Rate Splitting in FDD Massive MIMO Systems Based on the Second Order Statistics of Transmission Channels

In this work, we present new results for the application of rate splitting multiple access (RSMA) to the downlink (DL) of a massive multiple-input-multiple-output (MaMIMO) system operating in frequency-division-duplex (FDD) mode. Due to the lack of uplink (UL) - DL channel reciprocity in such systems, explicit training in the DL has to be performed in order to gain knowledge about the single-antenna users' channels at the base station (BS). This is ensured through a feedback link from the users to the BS. Dealing with the DL of a massive MIMO system implies that acquiring the DL channel state information (CSI) comes at the cost of a huge training overhead that scales with the number of BS antennas. Therefore, we limit the resources allocated to training by reusing the pilot sequences among the BS antennas that results in a contaminated channel observation. Despite this incomplete channel knowledge at the transmitter side, the proposed RS approach combined with a statistical precoder relying on the channels' second-order information achieves excellent results in terms of spectral efficiency compared to the state-of-art techniques. This is demonstrated via Monte-Carlo simulations of typical communication scenarios.

==> Conclusion.tex <==
In this work, we presented a framework for the application of rate splitting to an FDD massive multi-user MIMO system. Despite the suboptimality of the proposed approach and the incomplete channel knowledge at the BS, numerical results have shown that the combination of the bilinear precoding based on the second-order channel information and rate splitting leads to a drastic improvement in terms of the achievable sum rate when compared to the system without rate splitting. The transmission of the common message is mainly beneficial when it comes to medium to high transmit powers. While the conventional DL system (usual broadcast channel, without rate splitting) saturates in the high transmit power regime due to the inter-user interference and the imperfect channel knowledge, introducing the common stream yields a rate of the system that increases when more transmit power is used.  Furthermore, our method significantly outperforms the commonly used iterative weighted MMSE approach. While the optimization problem related to the latter has to be solved in each and every channel coherence interval, the bilinear approach depending on the channel covariance matrices requires a simple matrix-vector multiplication in every channel coherence interval. Finding the deterministic transformation matrices that constitute the bilinear precoder has only to be performed in the beginning of the covariance coherence interval which is given by several channel coherence intervals.\\
A future research direction would be to extend the proposed approach to a multi-cell setup where the challenges related to the system design become more significant due to the inter-cell interference. Furthermore, since the benefits of RS decrease as the number of served users increases, one could optimize the set of users that have to decode the common stream, which could increase the minimum common rate. This user selection can be based on the channel second-order statistics.

==> IWMMSE.tex <==
To compare the performance of the proposed approach, we briefly present the iterative weighted mean square error (IWMSE) precoding approach proposed in \cite{IWMMSE}. This method is based on establishing a relationship between the sum rate maximization problem and the augmented weighted MSE minimization problem by introducing weights and equalizing filters. The latter optimization problem turns out to be convex in each of its variables when the other ones are kept constant and hence an alternating solution approach is pursued. 

Let $g_{\tc,k}$ and $g_{\tp,k}$ be the equalizing filters for the $k$th user's common and private message, respectively. \\
Given the expressions in \eqref{eq:rck} and in \eqref{eq:rpk}, the estimates for the $k$th user common message and private message denoted respectively by $\hat{s}_{\tc,k}$  and $\hat{s}_{\tp,k}$ read as
\begin{align}
    &\hat{s}_{\tc,k}=g_{\tc,k} r_{\tc,k}= g_{\tc,k} \bs{h}_k^\HH \bs{p}_\tc s_\tc + g_{\tc,k} \sum_{j=1}^{K} \bs{h}_k^\HH \bs{p}_{\tp,j} s_{\tp,j} + g_{\tc,k} v_k\\
    &\hat{s}_{\tp,k}=g_k r_{\tp,k} = g_k \sum_{j=1}^{K} \bs{h}_k^\HH \bs{p}_{\tp,j} s_{\tp,j} + g_{\tc,k} v_k
\end{align}
The MSEs of the common message and the private message for user $k$ can be written as
\begin{align}
    &\varepsilon_{\tc,k}=\mathbb{E}[|\hat{s}_{\tc,k}-s_\tc|^2]=|g_{\tc,k}|^2\left(|\bs{h}_k^\HH \bs{p}_\tc|^2 + \sum_{j=1}^{K}  |\bs{h}_k^\HH \bs{p}_j|^2 + 1 \right) + 1 -2 \Re\{g_{\tc,k}^* \bs{p}_\tc^\HH \bs{h}_k\}\\
     &\varepsilon_{\tp,k}=\mathbb{E}[|\hat{s}_{\tp,k}-s_k|^2]=|g_{\tp,k}|^2\left( \sum_{j=1}^{K}  |\bs{h}_k^\HH \bs{p}_{\tp,j}|^2 + 1 \right) + 1 -2 \Re\{g_{\tp,k}^* \bs{p}_{\tp,k}^\HH \bs{h}_k\}.
\end{align}
Minimizing the MSEs with respect to the equalizing filters $g_{\tc,k}$ and $g_{\tp,k}$, yields the MMSE optimal filters 
\begin{equation}
    g_{\tc,k}^\text{MMSE}=\frac{\bs{p}_\tc^\HH \bs{h}_k}{T_{\tc,k}}, \qquad
     g_{\tp,k}^\text{MMSE}=\frac{\bs{p}_{\tp,k}^\HH \bs{h}_k}{T_{\tp,k}}
    \label{eq:gckgk}
\end{equation}
where $T_{\tc,k}= |\bs{h}_k^\HH \bs{p}_\tc|^2 + \sum_{j=1}^{K}  |\bs{h}_k^\HH \bs{p}_{\tp,j}|^2 + 1 $ and $T_{\tp,k}=\sum_{j=1}^{K}  |\bs{h}_k^\HH \bs{p}_{\tp,j}|^2 + 1 $.\\
Applying the MMSE equalizing filters from \eqref{eq:gckgk} yields the following MMSE expressions, which are closely related to the instantaneous common and private SINRs
\begin{equation}
   \varepsilon_{\tc,k}^\text{MMSE}=1-\frac{|\bs{h}_k^\HH \bs{p}_\tc|^2}{T_{\tc,k}}=\frac{1}{1+\gamma_{\tc,k}^\text{inst}}, \qquad
   \varepsilon_{\tp,k}^\text{MMSE}=1-\frac{|\bs{h}_k^\HH \bs{p}_{\tp,k}|^2}{T_{\tp,k}}=\frac{1}{1+\gamma_{\tp,k}^\text{inst}}.
    \label{eq:MMSEs}
\end{equation}
Now, introducing the common and private weights $u_{\tc,k}$ and $u_{\tp,k}$, we consider the augmented weighted MSEs
\begin{equation}
 \begin{aligned}
    &\xi_{\tc,k}=u_{\tc,k}\varepsilon_{\tc,k} - \log(u_{\tc,k})\\
    &\xi_{\tp,k}=u_{\tp,k}\varepsilon_{\tp,k} - \log(u_{\tp,k}).
\end{aligned}   
\label{eq:xick}
\end{equation}
When the MSEs are fixed, the optimal weights that minimize $\xi_{\tc,k}$ and $\xi_{\tp,k}$ are given by $u_{\tc,k}^*=1/\varepsilon_{\tc,k}$ and $u_{\tp,k}^*=1/\varepsilon_{\tp,k}$. \\
Note that by inserting these expressions into \eqref{eq:xick} and applying the MMSE equalizing filters yields the following augmented weighted MMSEs
\begin{equation}
    \xi_{\tc,k}^\text{MMSE}=1-R_{\tc,k}^\text{inst}, \quad  \xi_{\tp,k}^\text{MMSE}=1-R_{\tp,k}^\text{inst} \label{eq:XiRate}
\end{equation}
where $R_{\tc,k}^\text{inst}$ and $R_{\tp,k}^\text{inst}$ are the common and private rates of user $k$ respectively, given by $R_{\tc,k}^\text{inst}=\log_2(1+\gamma_{\tc,k}^\text{inst})$ and $R_{\tp,k}^\text{inst}=\log_2(1+\gamma_{\tp,k}^\text{inst})$.\\
The BS has only access to an estimate $\hat{\bs{H}}$ of the channel and therefore the instantaneous rates are not known to the BS. The authors define the average common and private rates of user $k$ $\bar{R}_{\tc,k}=\mathbb{E}[R_{\tc,k}^\text{inst}|\hat{\bs{H}}]$ and $\bar{R}_{\tp,k}=\mathbb{E}[R_{\tp,k}^\text{inst}|\hat{\bs{H}}]$, to which the BS has access. The average common rate is then given by $\bar{R}_\tc=\underset{k}{\min} \bar{R}_{\tc,k}$. The average sum rate maximization problem hence reads as
\begin{equation}
    \begin{aligned}
    \underset{\substack{\bar{R}_\tc,\bs{p}_\tc\\ \bs{p}_{\tp,1},\dots, \bs{p}_{\tp,K}}}{\max} \: &\bar{R}_\tc + \sum_{k=1}^K  \bar{R}_{\tp,k} \\
    &\text{s.t.} \quad \bar{R}_\tc\leq \bar{R}_{\tc,k}, \forall k\\
    &\|\bs{p}_\tc\|^2+\sum_{k=1}^K \|\bs{p}_{\tp,k}\|^2 \leq P_\text{dl}.
    \end{aligned}
    \label{eq:ASR}
\end{equation}
Note that contrarily to \eqref{eq:OptPrimal}, the optimization problem \eqref{eq:ASR} exhibits an instantaneous power constraint and has to be solved in every channel coherence interval. \\
Due to the intractability of \eqref{eq:ASR}, the authors deploy the so-called the sample average approximation (SAA) in order to evaluate the average rates. Given the channel estimate $\hat{\bs{h}}_k$ and the known error variance $\sigma_{e,k}^2$, the BS generates $N_s$ samples of the channel such that the $n$th sample is given by
\begin{equation*}
    \bs{h}_k^{(n)}=\sqrt{1-\sigma_{e,k}^2}\hat{\bs{h}}_k + \sqrt{\sigma_{e,k}^2} \tilde{\bs{h}}_k 
\end{equation*}
where $\tilde{\bs{h}}_k \sim \mathcal{N}_\mathbb{C}(\bs{0}, \bs{I}_M)$.\\ 
The average common and private rates are then approximated using these samples according to $\bar{R}_{\tc,k}^{(N_s)}=\frac{1}{N_s}\sum_{n=1}^{N_s}  R_{\tc,k}^\text{inst}(\bs{H}^{(n)})$ and $\bar{R}_{\tc,k}^{(N_s)}=\frac{1}{N_s}\sum_{n=1}^{N_s}  R_{\tp,k}^\text{inst}(\bs{H}^{(n)})$, respectively, with $\bs{H}^{(n)}=[\bs{h}_1^{(n)},\dots,\bs{h}_K^{(n)}]$.

Similar to \eqref{eq:XiRate}, a relationship between the approximated rates and the approximated augmented weighted MMSEs can be established
\begin{equation}
    \bar{\xi}_{\tc,k}^{\text{MMSE}(N_s)}=1-\bar{R}_{\tc,k}^{(N_s)}, \quad \bar{\xi}_{\tp,k}^{\text{MMSE}(N_s)}=1-\bar{R}_{\tp,k}^{(N_s)}
\end{equation}
where $\bar{\xi}_{\tc,k}^{\text{MMSE}(N_s)}=\frac{1}{N_s} \sum_{n=1}^{N_s} \xi_{\tc,k}^{\text{MMSE}}(\bs{H}^{(n)})$ and $\bar{\xi}_{\tp,k}^{\text{MMSE}(N_s)}=\frac{1}{N_s} \sum_{n=1}^{N_s} \xi_{\tp,k}^{\text{MMSE}}(\bs{H}^{(n)})$.

We can now formulate the optimization problem based on the approximated augmented weighted MSEs
\begin{equation}
    \begin{aligned}
    \underset{\substack{\bar{\xi}_\tc, \bs{U}, \bs{G}\\\bs{p}_\tc, \bs{p}_{\tp,1},\dots, \bs{p}_{\tp,K}}}{\min} \: & \xi_\tc + \sum_{k=1}^K \bar{\xi}_{\tp,k}^{\text{MMSE}(N_s)}\\
  \text{s.t.} \quad  &\bar{\xi}_\tc\geq \bar{\xi}_{\tc,k}^{\text{MMSE}(N_s)}, \forall k\\
    &\|\bs{p}_\tc\|^2+\sum_{k=1}^K \|\bs{p}_{\tp,k}\|^2 \leq P_\text{dl}
    \end{aligned}
    \label{eq:OptXi}
\end{equation}
where the weights and equalizing filters corresponding to the $N_s$ samples are collected respectively in $\bs{U}$ and $\bs{G}$.\\
The optimization problem \eqref{eq:OptXi} is convex in each of its blocks ($\bs{U}$, $\bs{G}$ and $\bs{P}=[\bs{p}_\tc, \bs{p}_1, \dots, \bs{p}_K]$) if the other two are fixed. Therefore, an alternating solution approach is used.\\
For fixed precoders, $\bs{U}$ and $\bs{G}$ are computed according to the MMSE solution as explained in the beginning of this section. The weights and equalizing filters are calculated for each of the $N_s$ samples and subsequently averaged out. Then, if $\bs{U}$ and $\bs{G}$ are fixed, the optimization problem reduces to a quadratically constrained convex problem which can be solved using standar
 
Note that the optimization problem in \eqref{eq:OptXi} exhibits the same structure as the sum rate maximization problem stated in \eqref{eq:OptPrimal}. The main difference lies in the fact, that \eqref{eq:OptXi} has to be solved in every channel coherence interval, since the optimization variables depend on the instantaneous channel knowledge. This also gives rise to the instantaneous power constraint. Additionally, the allocation of the power among the common and private stream transmission is performed implicitly, i.e., there is no explicit optimization over the common power fraction as in \eqref{eq:OptPrimal}.\\
To compute the MSE minimizing equalizing filters $g_{\tc,k}^\text{MMSE}$ and $g_k^\text{MMSE}$ and the weights $u_{\tc,k}^\text{MMSE}=1/\varepsilon_{\tc,k}^\text{MMSE}$ and $u_{k}^\text{MMSE}=1/\varepsilon_{k}^\text{MMSE}$, we use the MMSE channel estimate $\hat{\bs{h}}_k^\text{MMSE}$ that we obtain from the channel observation $\bs{y}_k$.  This is given by
\begin{align*}
    \hat{\bs{h}}_k^\text{MMSE}= \bs{C}_k \bs{\Phi} (\bs{\Phi}^\HH \bs{C}_k \bs{\Phi} + \sigma_n^2 \bs{I}_{T_\text{dl}})^{-1} \bs{y}_k.
\end{align*}
To tackle the augmented weighted MMSE problem in \eqref{eq:OptXi}, we again use the quadratic transform applied to fractional programming problems. The fractions are found inside the MMSE expressions [cf. \eqref{eq:MMSEs}]. By defining the auxiliary variables $w_{\tc,k}$ and $w_{\tp,k}$ associated with each of the fractions inside the common and private MMSE expressions as follows
\begin{equation}
    w_{\tc,k}=\frac{\bs{h}_k^\HH \bs{p}_\tc}{T_{\tc,k}}, \quad 
    w_{\tp,k}=\frac{\bs{h}_k^\HH \bs{p}_{\tp,k}}{T_{\tp,k}}
    \label{eq:AuxW}
\end{equation}
we can now reformulate the equivalent optimization problem to \eqref{eq:OptXi} using the quadratic transform
\begin{equation}
    \begin{aligned}
    \underset{\xi_\tc,\bs{P}}{\min} \: & \xi_\tc + \sum_{k=1}^K u_{\tp,k}^\text{MMSE} (1-2\Re\{w_{\tp,k}^* \bs{h}_k^\HH \bs{p}_{\tp,k}\} + |w_{\tp,k}|^2 T_{\tp,k} ) - \log_2(u_{\tp,k}^\text{MMSE})\\
     \text{s.t.} \quad &\xi_\tc\geq u_{\tc,k}^\text{MMSE} (1-2\Re\{w_{\tc,k}^* \bs{h}_k^\HH \bs{p}_\tc\} + |w_{\tc,k}|^2 T_{\tc,k} ) - \log_2(u_{\tc,k}^\text{MMSE}), \forall k\\
    &\text{tr}(\bs{P}\bs{P}^\HH) \leq P_\text{dl}
    \end{aligned}
    \label{eq:OptXi2}
\end{equation}
where we defined the precoding matrix $\bs{P}=[\bs{p}_\tc, \bs{p}_{\tp,1}, \dots, \bs{p}_{\tp,K}]$. \\
The optimization problem in \eqref{eq:OptXi2} is convex in $\xi_\tc$ and $\bs{P}$ and can therefore be solved using the CVX solver. Here, again, we need to alternate between solving \eqref{eq:OptXi2} for fixed auxiliary variables and updating those according to \eqref{eq:AuxW}. \\
The whole approach is summarized in Algorithm~\ref{alg:IWMMSE}.\\
\begin{algorithm}
\caption{Iterative Weighted MMSE Algorithm}\label{alg:IWMMSE}
\begin{algorithmic}[1]
\State Initialize: $\bs{p}_\tc=\sqrt{\alpha_\tc P_\text{dl}}\frac{\sum_{i=1}^K\hat{\bs{h}}_i}{\|\sum_{i=1}^K\hat{\bs{h}}_i\|_2}$ and $\bs{P}_\tp=\sqrt{(1-\alpha_\tc)P_\text{dl}}\frac{\hat{\bs{H}}}{\|\hat{\bs{H}}\|_F}$ where $\bs{P}_\tp=[\bs{p}_{\tp,1},\dots, \bs{p}_{\tp,K}]$ and $\hat{\bs{H}}=[\hat{\bs{h}}_1,\dots, \hat{\bs{h}}_K]$
\State Compute the MMSEs $\varepsilon_{\tc,k}^\text{MMSE}$ and $\varepsilon_{\tp,k}^\text{MMSE}$ giving the weights $u_{\tc,k}^\text{MMSE}$ and $u_{\tp,k}^\text{MMSE}$
\State Compute the auxiliary variables according to \eqref{eq:AuxW}.
\State Solve the optimization problem in \eqref{eq:OptXi2} via CVX
\State Alternate between steps 2--4 until convergence.
\end{algorithmic}
\end{algorithm}
